Reduktionssysteme zur Berechnung einer Aufl\"osung der orthogonalen freien Quantengruppen $A_o(n)$

F\"ur die freien orthogonalen Quantengruppen $A_o(n)$ wird ein vollst\"a ndiges Reduktionssystem angegeben und verifiziert. F\"ur den Fall $n = 2$ wird ein endlicher Automat angegeben, der s\"amtliche der Basiselemente findet. Weiterhin wird eine Basis f\"ur die f\"ur die Kerne einer freien Aufl\"osung von $A_o(n)$ als Bimodul bewiesen. Abschlie{\ss}end wird mit der nun verifizierten Aufl\"osung die Homologie von $A_o(n)$ explizit berechnet.

==> Haupt/RechnungAufloesung/Phi1.tex <==
\subsection{Reduktionswege für $a_{p,1}a_{q,1}e$}

%Ich lasse den Erzeuger $e$ vom Modul $\Algebra$ in der Rechnung stets weg. \\
%Konflikt mit $Z_{p,q}$:


\subsubsection{Beginnend mit $(a_{p,1}a_{q,1}e ~,~ Z_{p,q}e)$:}
\Gleichung{
\underline{a_{p,1}a_{q,1}e} \Pfeil{\widetilde{Z}_{p,q}}& -\Sum{i=2}a_{p,i}\underline{a_{q,i}e}+ \delta_{p,q}e\\
\Pfeil{\widetilde{V}_{q,i}} & -\Sum{i=2}a_{p,i}\delta_{q,i}e + \Sum{i=2}a_{p,i}e_{q,i} + \delta_{p,q}e\\
= & -(1-\delta_{q,1})\underline{a_{p,q}e}+ \Sum{i=2}a_{p,i}e_{q,i} + \delta_{p,q}e\\
\Pfeil{\widetilde{V}_{p,q}}& -(1-\delta_{q,1})\delta_{p,q}e + (1-\delta_{q,1})e_{p,q}+ \Sum{i=2}a_{p,i}e_{q,i} + \delta_{p,q}e\\
= &~ \delta_{q,1}\delta_{p,1}e + e_{p,q} - \delta_{q,1}e_{p,1}+ \Sum{i=2}a_{p,i}e_{q,i} 
}
\subsubsection{Beginnend mit $(a_{p,1}a_{q,1}e ~,~ V_{q,1}e)$:}
\Gleichung{
a_{p,1}\underline{a_{q,1}e} \Pfeil{\widetilde{V}_{q,1}}& a_{p,1}\delta_{q,1}e- a_{p,1}e_{q,1}\\
&=\delta_{q,1}\underline{a_{p,1}e} - \underline{a_{p,1}e_{q,1}}\\
 \Pfeil{\widetilde{V}_{p,1}, \widetilde{K}_{p,q}}& \delta_{q,1}\delta_{p,1}e-\delta_{q,1}e_{p,1}e  + \sum_{i=2}^n a_{p,i}e_{q,i}  + e_{p,q}
}

\Frage{Hier fehlen noch die anderen Konflikte}



==> Haupt/RechnungAufloesung/Phi2.tex <==
\subsection{Reduktionswege für $a_{n,n}e_{n,n} $}
\label{WV}

\subsubsection{Beginnend mit $(a_{n,n}e_{n,n} ~,~ W_{n,n})$:}
\Gleichung{
&\underline{a_{n,n}e_{n,n} } \\ 
	\Pfeil{\widetilde{W}_{n,n} } & -\SuM{j}\underline{a_{j,n}e_{j,n}}- e_{n,n} + \Sum{j=1}a_{j,n}f_{j,n}\\
	\Pfeil{\widetilde{V}_{j,j} } &\SuM{j}\SuM{i}a_{j,i}e_{j,i}+\SuM{j}e_{j,j} -\SuM{j} f_{j,j}
	- e_{n,n} + \SuM{j}a_{j,n}f_{j,n}
			\\&+ \underline{a_{n,n}f_{n,n}}\\
	%
	\Pfeil{\widetilde{K} } &\SuM{j}\SuM{i}a_{j,i}e_{j,i}+\SuM{j}e_{j,j} -\SuM{j} f_{j,j}
	- e_{n,n} + \SuM{j}a_{j,n}f_{j,n} \\&
	- \SuM{i,j}a_{j,i}f_{j,i} - \SuM{j}a_{j,n}f_{j,n}- \SuM{i}a_{n,i}f_{n,i} + \Sum{i=1}f_{i,i}
	\\
	=&\SuM{j}\SuM{i}a_{j,i}e_{j,i}+\SuM{j}e_{j,j} 
	- e_{n,n}  \\&
	- \SuM{i,j}a_{j,i}f_{j,i} - \SuM{i}a_{n,i}f_{n,i} + f_{n,n}
}%Geleichung

 

\subsubsection{Beginnend mit $(a_{n,n}e_{n,n} ~,~ V_{n,n})$:}
\Gleichung{
\underline{a_{n,n}e_{n,n}} ~ 
	\Pfeil{\widetilde{V}_{n,n} } & -\SuM{i}\underline{a_{n,i}e_{n,i}}- e_{n,n} + f_{n,n}\\
	\Pfeil{\widetilde{W}_{i,i} } & \SuM{i}\SuM{j}a_{j,i}e_{j,i}+\SuM{i} e_{i,i} -\SuM{i} \Sum{j=1}a_{j,i}f_{j,i}- e_{n,n} + f_{n,n}\\
	=&\SuM{j}\SuM{i}a_{j,i}e_{j,i}+\SuM{j}e_{j,j} 
	- e_{n,n}  \\&
	- \SuM{i,j}a_{j,i}f_{j,i} - \SuM{i}a_{n,i}f_{n,i} + f_{n,n}
}%Geleichung





\newpage









\subsection{Reduktionswege für $a_{p,1}a_{n,1}e_{n,q}$}
\label{ZiW}

\subsubsection{Beginnend mit $(a_{p,1}a_{n,1}e_{n,q} ~,~ Z_{p,n}e_{n,q})$:}
\Gleichung{
&\underline{a_{p,1}a_{n,1} }e_{n,q}  \\
	\Pfeil{\widetilde{Z}_{p,n} } & - \Sum{i=2}a_{p,i}\underline{a_{n,i} e_{n,q}}+  \delta_{p,n} e_{n,q}\\
	%
	\Pfeil{\widetilde{W}_{i,q} } &   \Sum{i=2}a_{p,i}\left( \SuM{j}a_{j,i}e_{j,q}+ e_{q,i} -  \Sum{j=1}a_{j,i}f_{j,q}\right) + \delta_{p,n} e_{n,q}\\
	%
	=&  \SuM{j}\Sum{i=1}a_{p,i}a_{j,i}e_{j,q} + \sum_{i=2}^{n-1}a_{p,i}e_{q,i} + \underline{a_{p,n}e_{q,n}} + \delta_{p,n} e_{p,q}\\
	&- \Sum{i=2}\Sum{j=1} a_{p,i} a_{j,i}f_{j,q}\\
	%
		\Pfeil{\widetilde{V}_{p,q} }&  \SuM{j}\Sum{i=2}a_{p,i}a_{j,i}e_{j,q} + \sum_{i=2}^{n-1}a_{p,i}e_{q,i}  -\SuM{i}a_{p,i}e_{q,i}\\&
		- e_{p,q} + f_{p,q}+ \delta_{p,n} e_{p,q}-\Sum{i=2}\Sum{j=1} a_{p,i} a_{j,i}f_{j,q} \\
		%
		=&  -\SuM{j}\left(Z_{p,j}-\delta_{p,j}\right)e_{j,q} -a_{p,1}e_{q,1}
		-(1-\delta_{p,n}) e_{p,q} \\&+\Sum{j=1}\left(Z_{p,j}-\delta_{p,j}\right)f_{j,q} + f_{p,q}\\
		%
		%\NeueSeite
		=&  -\SuM{j}Z_{p,j}e_{j,q} -a_{p,1}e_{q,1} +\Sum{j=1}Z_{p,j}f_{j,q} \\
}%Geleichung

\subsubsection{Beginnend mit $(a_{p,1}a_{n,1}e_{n,q} ~,~ a_{p,1}W_{1,q})$:}
\Gleichung{
a_{p,1}\underline{ a_{n,1}e_{n,q}} ~ 
	\Pfeil{\widetilde{W}_{1,q} } & -\SuM{j}\underline{a_{p,1} a_{j,1}}e_{j,q}- a_{p,1}e_{q,1}
	+ \Sum{j=1}\underline{a_{p,1}a_{j,1}}f_{j,q}\\
	\Pfeil{\widetilde{Z}_{p,j},\widetilde{Z}_{p,j}  } & -\SuM{j} Z_{p,j}e_{j,q} - a_{p,1}e_{q,1}+ \Sum{j=1}Z_{p,j}f_{j,q}\\
%	=& \SuM{j} \Sum{i=2}a_{p,i} a_{j,i}e_{j,q} -(1- \delta_{p,n}) e_{p,q} - a_{p,1}e_{q,1} + a_{p,1}\Sum{j=1}f_{j,j}\\
}%Geleichung





\newpage





\subsection{Reduktionswege für $ a_{1,p}a_{1,n}e_{q,n}$}
\label{SiV}



\subsubsection{Beginnend mit $(a_{1,p}a_{1,n}e_{q,n} ~,~ S_{p,n}e_{q,n})$:}
\Gleichung{
&\underline{a_{1,p}a_{1,n} } e_{q,n}~ \\
	\Pfeil{\widetilde{S}_{p,n} } & - \Sum{j=2}a_{j,p}\underline{a_{j,n}e_{q,n}} + \delta_{p,n}e_{q,n}\\
	\Pfeil{\widetilde{V}_{j,q} } & \Sum{j=2}a_{j,p}\SuM{i}a_{j,i}e_{q,i}+\Sum{j=2}a_{j,p} e_{j,q} -\Sum{j=2}a_{j,p} f_{j,q}
																	+ \delta_{p,n}e_{q,n}\\
  =&\Sum{j=2}\SuM{i}a_{j,p}a_{j,i}e_{q,i} +\sum_{j=2}^{n-1}a_{j,p}e_{j,q}+\underline{a_{n,p}e_{n,q}}+ \delta_{p,n}e_{q,n}
     \\& -\Sum{j=2}a_{j,p} f_{j,q}	\\
%	
	\Pfeil{\widetilde{W}_{p,q} } & \Sum{j=2}\SuM{i}a_{j,p}a_{j,i}e_{q,i}  +\sum_{j=2}^{n-1}a_{j,p}e_{j,q}\\&-\SuM{j}a_{j,p}e_{j,q}- e_{q,p} + \Sum{j=1}a_{j,p}f_{j,q}
  			+ \delta_{p,n}e_{q,n}	-\Sum{j=2}a_{j,p} f_{j,q}\\
%
 =&	\Sum{j=2}\SuM{i}a_{j,p}a_{j,i}e_{q,i}  -a_{1,p}e_{1,q}- (1-\delta_{p,n})e_{q,p}	+a_{1,p} f_{1,q}										
}%Geleichung



\subsubsection{Beginnend mit $(a_{1,p}a_{1,n}e_{q,n} ~,~ a_{1,p}V_{1,q})$:}
\Gleichung{
&a_{1,p}\underline{a_{1,n}e_{q,n} } \\
	\Pfeil{\widetilde{V}_{1,q} } &  -\SuM{i}\underline{a_{1,p}a_{1,i}}e_{q,i}- a_{1,p}e_{1,q} + a_{1,p}f_{1,q}	\\
	\Pfeil{\widetilde{S}_{p,i} } &  \SuM{i}\Sum{j=2}a_{j,p}a_{j,i}e_{q,i} -  \SuM{i}\delta_{p,i}e_{q,i}
																  - a_{1,p}e_{1,q} + a_{1,p}f_{1,q}\\
	=& 	\SuM{i}\Sum{j=2}a_{j,p}a_{j,i}e_{q,i} -  (1-\delta_{p,n})e_{q,p} - a_{1,p}e_{1,q} + a_{1,p}f_{1,q}
}%Geleichung





\newpage



\subsection{Reduktionswege für $a_{p,1}a_{q,2}a_{n,2}e_{n,r}$}
\label{ZiiW}

\subsubsection{Beginnend mit $(a_{p,1}a_{q,2}a_{n,2}e_{n,r} ~,~ \left(Z_{p,q,n} - Z_{p,q}a_{n,1}\right) e_{n,r})$:}
\Gleichung{
&\underline{a_{p,1}a_{q,2}a_{n,2} }e_{n,r} ~ \\
	\Pfeil{\widetilde{Z}_{p,q,n} } & -\Sum{i=3} a_{p,1} a_{q,i}\underline{a_{n,i} e_{n,r}} + a_{p,1}\delta_{q,n}e_{n,r}  		-Z_{p,q}%\left(\Sum{i=2}a_{p,i}a_{q,i}  - \delta_{p,q}\right)
	\underline{a_{n,1}e_{n,r}} \\
	%
	\Pfeil{\widetilde{W}_{i,r},\widetilde{W}_{1,r}} & \Sum{i=3} a_{p,1} a_{q,i}\left(\SuM{j}a_{j,i}e_{j,r}+ e_{r,i} - \Sum{j=1}a_{j,i}f_{j,r}\right) \\&+ a_{p,1}\delta_{q,n}e_{n,r}
	 +Z_{p,q}%- \left(\Sum{i=2}a_{p,i}a_{q,i}  - \delta_{p,q}\right) 
	\left(\SuM{j}a_{j,1}e_{j,r}+ e_{r,1} - \Sum{j=1}a_{j,1}f_{j,r}\right) \\
	%
	=& \Sum{i=3}\SuM{j} a_{p,1} a_{q,i}a_{j,i}e_{j,r}+ \sum_{i=3}^{n-1} a_{p,1} a_{q,i}e_{r,i}	+a_{p,1} \underline{a_{q,n}e_{r,n}}  \\
	& + a_{p,1}\delta_{q,n}e_{n,r} 
	+Z_{p,q}%- \left(\Sum{i=2}a_{p,i}a_{q,i}  - \delta_{p,q}\right) 
	\left(\SuM{j}a_{j,1}e_{j,r}+ e_{r,1} \right) \\
	 & - \Sum{i=3}\Sum{j=1} a_{p,1} a_{q,i}a_{j,i}f_{j,r}  
	 -Z_{p,q}%+ \Sum{i=2}a_{p,i}a_{q,i}\Sum{j=1}a_{j,1}f_{j,r}  - \delta_{p,q}
	   \Sum{j=1}a_{j,1}f_{j,r}\\
	 %
\Pfeil{\widetilde{V}_{q,r}}& \Sum{i=3}\SuM{j} a_{p,1} a_{q,i}a_{j,i}e_{j,r}+ \sum_{i=3}^{n-1} a_{p,1} a_{q,i}e_{r,i}	\\
&	 -\SuM{i}a_{p,1} a_{q,i}e_{r,i} - a_{p,1}e_{q,r} +a_{p,1}f_{q,r} \\
	& + a_{p,1}\delta_{q,n}e_{n,r} 
	+Z_{p,q}%- \left(\Sum{i=2}a_{p,i}a_{q,i}  - \delta_{p,q}\right)
	 \left(\SuM{j}a_{j,1}e_{j,r}+ e_{r,1} \right) \\
	& - \Sum{i=3}\Sum{j=1} a_{p,1} a_{q,i}a_{j,i}f_{j,r}  	
	 -Z_{p,q}%+ \Sum{i=2}a_{p,i}a_{q,i}\Sum{j=1}a_{j,1}f_{j,r}  - \delta_{p,q}
	   \Sum{j=1}a_{j,1}f_{j,r}\\
	 %
	 =&\Sum{i=3}\SuM{j} a_{p,1} a_{q,i}a_{j,i}e_{j,r} -a_{p,1} a_{q,2}e_{r,2} - \underline{a_{p,1} a_{q,1}}e_{r,1} \\&
	 - (1-\delta_{q,n})a_{p,1}e_{q,r}   
	+Z_{p,q}\SuM{j}a_{j,1}e_{j,r}+ Z_{p,q}e_{r,1}  \\
	 & + a_{p,1}f_{q,r}- \Sum{i=3}\Sum{j=1} a_{p,1} a_{q,i}a_{j,i}f_{j,r}  	
	 -Z_{p,q}%+ \Sum{i=2}a_{p,i}a_{q,i}\Sum{j=1}a_{j,1}f_{j,r}  - \delta_{p,q}
	   \Sum{j=1}a_{j,1}f_{j,r}
	 %
	  \NeueSeite
	 \Pfeil{\widetilde{Z}_{p,q}} &\Sum{i=3}\SuM{j} a_{p,1} a_{q,i}a_{j,i}e_{j,r} -a_{p,1} a_{q,2}e_{r,2}  \\&
	- (1-\delta_{q,n})a_{p,1}e_{q,r}   
	+Z_{p,q}\SuM{j}a_{j,1}e_{j,r}  \\
	 & + a_{p,1}f_{q,r}- \Sum{i=3}\Sum{j=1} a_{p,1} a_{q,i}a_{j,i}f_{j,r}  	
	 -Z_{p,q}%+ \Sum{i=2}a_{p,i}a_{q,i}\Sum{j=1}a_{j,1}f_{j,r}  - \delta_{p,q}
	   \Sum{j=1}a_{j,1}f_{j,r}\\
}%Geleichung



\subsubsection{Beginnend mit $(a_{p,1}a_{q,2}a_{n,2}e_{n,r} ~,~ a_{1,p}a_{q,2}W_{2,r})$:}
\Gleichung{
&a_{p,1}a_{q,2}\underline{ a_{n,2}e_{n,r}} ~ \\
	\Pfeil{\widetilde{W}_{2,r} } &  -\SuM{j}\underline{a_{p,1}a_{q,2}a_{j,2}}e_{j,r} - a_{p,1}a_{q,2}e_{r,2} 
	+\Sum{j=1} \underline{a_{p,1}a_{q,2}a_{j,2}}f_{j,r}\\
	%
	\Pfeil{\widetilde{Z}_{p,q,j},\widetilde{Z}_{p,q,j}} & \SuM{j}\left( \Sum{i=3} a_{p,1} a_{q,i}a_{j,i} e_{j,r} - a_{p,1}\delta_{q,j}e_{j,r}  +  Z_{p,q} a_{j,1}e_{j,r}\right) 
	\\& - a_{p,1}a_{q,2}e_{r,2} \\&
	 -\Sum{j=1}\left(\Sum{i=3} a_{p,1} a_{q,i}a_{j,i}f_{j,r} + a_{p,1}\delta_{q,j}f_{j,r} -  Z_{p,q} a_{j,1} f_{j,r}\right)
	 %
	\\ =&\SuM{j} \Sum{i=3} a_{p,1} a_{q,i}a_{j,i} e_{j,r} - (1-\delta_{q,n})a_{p,1}e_{q,r}  
	\\&+  \SuM{j}Z_{p,q} a_{j,1}e_{j,r} 
 - a_{p,1}a_{q,2}e_{r,2} \\&
	 -\Sum{j=1}\Sum{i=3} a_{p,1} a_{q,i}a_{j,i}f_{j,r} + a_{p,1}f_{q,r} -  \Sum{j=1}Z_{p,q} a_{j,1} f_{j,r}
}%Geleichung
\newpage






\newpage






\subsection{Reduktionswege für $a_{1,p}a_{2,q}a_{2,n}e_{r,n} $}
\label{SiiV}

\subsubsection{Beginnend mit $(a_{1,p}a_{2,q}a_{2,n}e_{r,n} ~,~ \left(S_{p,q,n}- S_{p,q}a_{1,n}\right)e_{r,n})$:}
\Gleichung{
&\underline{a_{1,p}a_{2,q}a_{2,n} }e_{r,n} ~ \\
	\Pfeil{\widetilde{S}_{p,q,n} } & -\Sum{j=3}a_{1,p}a_{j,q}\underline{a_{j,n}e_{r,n}} + a_{1,p}\delta_{q,n}e_{r,n} 	
	-S_{p,q}%+\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
	\underline{a_{1,n}e_{r,n}}\\
	%
	\Pfeil{\widetilde{V}_{j,r},\widetilde{V}_{1,r} }& \Sum{j=3}a_{1,p}a_{j,q}\left(\SuM{i}a_{j,i}e_{r,i}+ e_{j,r} -  f_{j,r}\right) + a_{1,p}\delta_{q,n}e_{r,n}\\&
	+S_{p,q}%-\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
	\left( \SuM{i}a_{1,i}e_{r,i}- e_{1,r} + f_{1,r}\right)	\\
	%
	=& \Sum{j=3}\SuM{i}a_{1,p}a_{j,q}a_{j,i}e_{r,i}+ \sum_{j=3}^{n-1}a_{1,p}a_{j,q}e_{j,r} +\underline{a_{n,q}e_{n,r}}\\&
	+ \delta_{q,n}a_{1,p}e_{r,q}
	+S_{p,q}%-\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
	\left( \SuM{i}a_{1,i}e_{r,i}- e_{1,r} \right)	\\&
	-  \Sum{j=3}a_{1,p}a_{j,q}f_{j,r} 
	+S_{p,q}%-\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
	f_{1,r}\\
	%
	\Pfeil{\widetilde{W}_{p,q} } & \Sum{j=3}\SuM{i}a_{1,p}a_{j,q}a_{j,i}e_{r,i}+ \sum_{j=3}^{n-1}a_{1,p}a_{j,q}e_{j,r}\\&
	 -\SuM{j}a_{1,p}a_{j,q}e_{j,r}- a_{1,p}e_{r,q} + \Sum{j=1}a_{1,p}a_{j,q}f_{j,r}
	\\&
	+ \delta_{q,n}a_{1,p}e_{r,q}
	+S_{p,q}%-\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
	\left( \SuM{i}a_{1,i}e_{r,i}- e_{1,r} \right)	\\&
	-  \Sum{j=3}a_{1,p}a_{j,q}f_{j,r} 
	+S_{p,q}%-\left( \Sum{j=2}a_{j,p}a_{j,q} - \delta_{p,q}\right)
		f_{1,r}\\
		%
	=& \Sum{j=3}\SuM{i}a_{1,p}a_{j,q}a_{j,i}e_{r,i}- \underline{a_{1,p}a_{1,q}}e_{1,r}-a_{1,p}a_{2,q}e_{2,r}
	\\&	-(1- \delta_{q,n})a_{1,p}e_{r,q}
	+S_{p,q} \SuM{i}a_{1,i}e_{r,i}- S_{p,q}e_{1,r} 	\\&
	 +\underline{a_{1,p}a_{1,q}}f_{1,r}+a_{1,p}a_{2,q}f_{2,r}
	 +S_{p,q}	 	f_{1,r}\\
	 %
	 		\NeueSeite
\\	\Pfeil{\widetilde{S}_{p,q},\widetilde{S}_{p,q} } &\Sum{j=3}\SuM{i}a_{1,p}a_{j,q}a_{j,i}e_{r,i}-a_{1,p}a_{2,q}e_{2,r}
		-(1- \delta_{q,n})a_{1,p}e_{r,q}\\&
	+S_{p,q} \SuM{i}a_{1,i}e_{r,i} 
	 +a_{1,p}a_{2,q}f_{2,r}	
}%Geleichung


\subsubsection{Beginnend mit $(a_{1,p}a_{2,q}a_{2,n}e_{r,n} ~,~ a_{1,p}a_{2,q}V_{2,r})$:}
\Gleichung{
&a_{1,p}a_{2,q}\underline{a_{2,n}e_{r,n} } \\ 
	\Pfeil{\widetilde{V}_{2,r} } &  -\SuM{i}\underline{a_{1,p}a_{2,q}a_{2,i}}e_{r,i}- a_{1,p}a_{2,q}e_{2,r} + a_{1,p}a_{2,q}f_{2,r}	\\
	%
	\Pfeil{\widetilde{S}_{p,q,i} }& \SuM{i}\Sum{j=3}a_{1,p}a_{j,q}a_{j,i}e_{r,i} -\SuM{i} a_{1,p}\delta_{q,i}e_{r,i}\\& +\SuM{i} S_{p,q}a_{1,i}e_{r,i} 
	\\&- a_{1,p}a_{2,q}e_{2,r} + a_{1,p}a_{2,q}f_{2,r}	\\
	%
	=& \SuM{i}\Sum{j=3}a_{1,p}a_{j,q}a_{j,i}e_{r,i} - a_{1,p}a_{2,q}e_{2,r}- (1-\delta_{q,n})a_{1,p}e_{r,q} \\&+\SuM{i} S_{p,q}a_{1,i}e_{r,i} 	 + a_{1,p}a_{2,q}f_{2,r}
}%Geleichung
\newpage







==> Haupt/RechnungGBA/MusterRechnung.tex <==
\subsection{Reduktionswege für $ $}
\label{SiZil}

\subsubsection{Beginnend mit $( ~,~ )$:}
\Gleichung{
\underline{ } ~ 
	\Pfeil{\widetilde{}_{} } & 
}%Geleichung



\subsubsection{Beginnend mit $( ~,~ )$:}
\Gleichung{
\underline{ } ~ 
	\Pfeil{\widetilde{}_{} } & 
}%Geleichung



==> Titel/Abstract.tex <==
Hier fehlt noch Danksagung



\Frage{Vorstellung von Redukionssystemen.

-Warum ist die Freie Quanten-Gruppe interessant?

Berechnung der Gröbnerbasis von $A^n$. 

Mit Beispiel $A^2$.

Methode zur Berechnung des Kerns mit Verbesserung für den nicht kommutativen Fall.

Berechnung einer freien Auflösung.

Hochschildhomologie?\\

Die $l^2$-Homologie einer Algebra kann man mittels einer (möglichst minimalen) freien Auflösung berechnen. 
Es in manchen Fällen gibt es einen auf Reduktionssystemen basierenden Algorithmus zur Berechnung einer Auflösung.

Dieser Algorithmus wird vorgestellt (Newmann und Bergmann-Diamanden Lemma) und anschließend eine Auflösung für die freie Quantengruppe verifiziert.

Außerdem wird eine Normaldarstellung der Elemente der Freien Quantengruppe in der Freien Algebra angegeben und untersucht ob diese Algebra Nullteilerfrei ist.

}




==> Titel/Danksagung.tex <==


 Bedanken möchte ich mich beim Graduiertenkolleg "`Gruppen und Geometrie"' für die finanzielle Unterstützung meiner Promotion.
Anselm Knebusch danke ich für seine Bereitschaft, bei meinen Rechnungen Hilfestellung zu leisten.
Besonders möchte ich mich bei Andreas Lochmann für seine Unterstützung mit seinem Wissen zu Ordnungen bedanken. Ivan Yudin schulde ich tiefen 
Dank für seinen Beistand während des gesamten Zeitraumes und seine hilfreichen Ratschläge.

==> Titel/Deckblatt.tex <==
Hier fehlt das Deckblatt. 
